COOT: Cooperative Hierarchical Transformer for Video-Text Representation Learning

Many real-world video-text tasks involve different levels of granularity, such as frames and words, clip and sentences or videos and paragraphs, each with distinct semantics. In this paper, we propose a Cooperative hierarchical Transformer (COOT) to leverage this hierarchy information and model the interactions between different levels of granularity and different modalities. The method consists of three major components: an attention-aware feature aggregation layer, which leverages the local temporal context (intra-level, e.g., within a clip), a contextual transformer to learn the interactions between low-level and high-level semantics (inter-level, e.g. clip-video, sentence-paragraph), and a cross-modal cycle-consistency loss to connect video and text. The resulting method compares favorably to the state of the art on several benchmarks while having few parameters. All code is available open-source at https://github.com/gingsi/coot-videotext

==> tables_main/didemo.tex <==
% ---------- UNUSED ----------
\iffalse
\begin{table}[t]
    \caption{Video-paragraph retrieval results on AcitvityNet-captions dataset (val1 test-split).}\vspace{5pt}
    \centering
    \footnotesize
    \resizebox{1\columnwidth}{!}{
    \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{l c c c c  | c c c c }
        \toprule
  \multicolumn{1}{c}{} & 
  \multicolumn{4}{c}{Paragraph$\implies$Video} &
  \multicolumn{4}{c}{Video$\implies$Paragraph}   \\
  
  \cmidrule(r){2-5}
  \cmidrule(r){6-9}

  Method       &R$@$1 &R$@$5 &R$@$50 & MR  & R$@$1 &R$@$5 & R$@$50 & MR  \\
  \midrule
   LSTM-YT~\cite{venugopalan2015sequence}       & 0.0 & 4.0 & 24.0 & 102.0 & 0.0 & 7.0 & 38.0 & 98.0    \\ 
   No Context~\cite{venugopalan2014translating}    & 5.0 & 14.0 & 32.0 & 78.0 & 7.0 & 18.0 & 45.0 & 56.0   \\
   DENSE~\cite{krishna2017dense}         & 14.0 & 32.0 & 65.0 & 34.0 & 18.0 & 36.0 & 74.0 & 32.0  \\
   VSE~\cite{NIPS2013_5204}(~\cite{Shao_2018_ECCV})         & 11.7 & 34.7 & 85.7 & 10 & - & - & - & -  \\
   FIFO~\cite{Shao_2018_ECCV}         & 14.1 & 37.1 & - & - & - & - & - & -  \\
   FSE~\cite{cmhse}           & 18.2 & 44.8 & 89.1 & 7       & 16.7  & 43.1 &  88.4  & $7$   \\
   HSE~\cite{cmhse}    & 44.4\std{0.5} & 76.7\std{0.3} & 97.1\std{0.1} & 2.0 & 44.2\std{0.6} & 76.7\std{0.3} & 97.0\std{0.3} & 2.0 \\ 
   CE            & $ 18.2_{\pm0.3}$	& $47.7_{\pm0.6}$	& $91.4_{\pm0.4}$	& $6_{\pm0}$& $17.7_{\pm0.6}$	& $ 46.6_{\pm0.7}$	& $90.9_{\pm0.2}$	& $6_{\pm0}$     \\ \hline
   COOT$_{Lite}$ & \textbf{49.6\std{0.4}} & \textbf{82.2\std{0.2}} & \textbf{98.1\std{0.2}} & ? & \textbf{51.4\std{0.2}}  & \textbf{82.7\std{0.3}} & \textbf{98.1\std{0.2}}   & ?    \\ 
   COOT$_{big}$  & \textbf{53.8\std{0.1}} & \textbf{84.5\std{0.5}} & \textbf{98.3\std{0.1}} & ? & \textbf{54.6\std{0.2}}  & \textbf{84.8\std{0.1}} & \textbf{98.4\std{0}}   & ?    \\ 
   

  \bottomrule\\[-20pt]
\end{tabular}}
\label{tab:ablate-attention_size}
\end{table}
\fi
